Predicting Signed Edges with $O(n^{1+o(1)} \log{n})$ Queries

Social networks and interactions in social media involve both positive and negative relationships. Signed graphs capture both types of relationships: positive edges correspond to pairs of "friends", and negative edges to pairs of "foes". The {\em edge sign prediction problem}, which aims to predict whether an interaction between a pair of nodes will be positive or negative, is an important graph mining task for which many heuristics have recently been proposed \cite{leskovec2010predicting,leskovec2010signed}. Motivated by social balance theory, we model the edge sign prediction problem as a noisy correlation clustering problem with two clusters. We are allowed to query each pair of nodes whether they belong to the same cluster or not, but the answer to the query is corrupted with some probability $0<q<\frac{1}{2}$. Let $c=\frac{1}{2}-q$ be the gap. We provide an algorithm that recovers the clustering with high probability in the presence of noise for any constant gap $c$ with $O(n^{1+\tfrac{1}{\log\log{n}}}\log{n})$ queries. Our algorithm uses simple breadth first search as its main algorithmic primitive. Finally, we provide a novel generalization to $k \geq 3$ clusters and prove that our techniques can recover the clustering if the gap is constant in this generalized setting.

==> Algorithms.tex <==
We prove our main result through a sequence of claims and lemmas. At a high level, our proof strategy is as follows: 

\begin{enumerate} 
\item We compute the probability that an edge disjoint path provides us with the correct information on whether $f(u)=f(v)$ or not. See Claim~\ref{claim1}.  
\smallskip
\item We show that there exist $N=e^{\tfrac{4\log{n}}{5\sqrt{\log\log{n}}}}$ almost edge-disjoint paths of length $(1+o(1))\diam$ between any pair of vertices with probability at least $1-\frac{1}{n^3}$. See Lemmas~\ref{lem1},\ref{lem2},~\ref{lem4}. 
\smallskip
\item  For each path from the collection of $N$ almost edge disjoint paths, we compute the product of the sign of the edges along the path. Since the paths are almost edge disjoint, the corresponding random variables are weakly dependent. We use concentration of multivariate polynomials \cite{gavinsky2014tail}, see also \cite{alonspencer,kim-vu}, in combination with Claim~\ref{claim1} to show that using the majority of the $N$ resulting signs to decide whether $f(u)=f(v)$ or not for a pair of nodes $u,v \in V(G)$ is lower bounded by $1-\frac{1}{n^3}$. Taking the union bound over ${n \choose 2}$ pairs concludes the proof. This is shown in Lemma~\ref{lem5}.
\end{enumerate}

The pseudocode is shown as Algorithm~\ref{alg:2cc}. The algorithm invokes for each pair of nodes   Algorithm~\ref{alg:edgeDisjointPaths} that constructs almost edge disjoint paths for each pair of nodes using Breadth First Search. Using appropriate data structures, Algorithm~\ref{alg:2cc} runs in time is $O(n^2(n+m))=O(n^3\log{n})$, where $n,m=20n\log{n}$ is the number of nodes and edges respectively.

\begin{algorithm}[t]
\caption{\label{alg:2cc} 2-Correlation Clustering with Noise} 
 \begin{algorithmic} 
\STATE Perform $20n\log{n}$ queries uniformly at random.
\STATE Let $G(V,E,\f)$ be the resulting graph, $\f:E\rightarrow \{+1,-1\}$ 
 \FOR{each item pair $u,v$} 
 \STATE {$\mathcal{P}_{u,v}=\{P_1,\ldots,P_r\}$ Edge-Disjoint-Paths($u,v$)}  
 \STATE  $Y_i \leftarrow \prod_{e \in P_i} \f(e)$ for $i=1,\ldots,r$  
 \STATE $Y_{uv} \leftarrow \sum_{P \in \mathcal{P}_{u,v}} Y_P $
  \IF{$Y_{uv} \geq 0$} 
  \STATE {$\f(u) = \f(v)$} 
  \ELSE 
  \STATE{$\f(u)\neq \f(v)$} 
  \ENDIF
 \ENDFOR


\STATE For each item pair $u,v$ run
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{\label{alg:edgeDisjointPaths}  Edge-Disjoint-Paths($u,v$)} 
 \begin{algorithmic}  
\REQUIRE $G(V,E,\f)$, $u,v \in V(G)$ 
\STATE $\epsilon \leftarrow \frac{1}{\sqrt{\log\log{n}}}$
\STATE Using Breadth First Search (BFS) grow a tree $T_u$ starting from $u$ with branching factor $4\log{n}$ until it reaches depth equal to $\epsilon L$. Similarly, grow a tree $T_v$ rooted at $v$, node disjoint from $T_u$ of equal depth.
\STATE From each leaf $u_i$ ($v_i$) of  $T_u$ ($T_v$) 
grow  node disjoint trees until they reach depth $(\frac{1}{2}+\epsilon)L$.  Finally, find an edge between $T_{u_i},T_{v_i}$ 
\end{algorithmic}
\end{algorithm}



\begin{claim} 
\label{claim1} 
Consider a  path $P_{uv}$ between nodes $u,v$ of length $L$. Let $R_{uv}=\prod_{e \in P_{uv}} \f(e)$. Then, 
\begin{equation}
\label{eq1} 
\Prob{R_{uv}=1} = \frac{1+(1-2q)^L}{2}.
\end{equation}
\end{claim} 
 
\begin{proof} 
Notice that $R_{uv} = 1$ iff $\f$ agrees with the unknown clustering function $f$ on $u,v$. This happens when the number of corrupted edges along that path $P_{uv}$ is even. Let $Z_{uv} \sim Bin(L,q)$
be the number of corrupted edges/sign flips along the $P_{uv}$ path.
Clearly, $\Prob{Z_{uv}=\text{even}}+ \Prob{Z_{uv}=\text{odd}}=1$. Also,

\begin{align*}
(1-2q)^L = ((1-q)-q)^L &= \sum_{k=0}^L {L \choose k} (-q)^k (1-q)^{L-k}   \\ 
&=  \sum_{k=0}^{\lfloor \frac{L}{2} \rfloor } {L \choose 2k} q^{2k} (1-q)^{L-2k} - \sum_{k=0}^{\lfloor \frac{L}{2} \rfloor }  {L \choose 2k+1} q^{2k+1} (1-q)^{L-(2k+1)} \\
&= \Prob{Z_{uv}=\text{even}}- \Prob{Z_{uv}=\text{odd}}.
\end{align*} 
By combining the above equations, we obtain that $\Prob{R_{uv}=1} =\Prob{Z_{uv}=\text{even}}= \frac{1+(1-2q)^L}{2}$.
\end{proof}

\noindent  Notice that since we perform $20n\log{n}$ queries uniformly at random, the resulting graph is asymptotically equivalent to $G \sim G(n,\frac{20\log{n}}{n})$.  Here, $G(n,p)$ is the classic Erd\"{o}s-R\'{e}nyi model  or random binomial graph model where each possible edge between each pair  $(u,v) \in {[n] \choose 2}$ is included in the graph with probability $p$ independent from every other edge.  
The diameter of this graph \whp grows as $\diam$ \cite{bollobas}. 
The next lemma is a direct corollary of the lower tail multiplicative Chernoff bound. 


\begin{lemma} 
\label{lem1} 
Let $G \sim G(n,\frac{20\log{n}}{n})$ be a random binomial graph. Then \whp all vertices have degree greater than $5\log{n}$. 
\end{lemma} 

\begin{proof} 
The degree $deg(u)$ of a node $u \in V(G)$ follows the binomial distribution $Bin(n-1,\frac{20\log{n}}{n})$. Set $\delta = \frac{3}{4}$. Then 

\begin{align*}
\Prob{  deg(u) <5 \log{n}  } &< e^{- \frac{\delta^2}{2} 20\log{n} }  \ll n^{-1}.
\end{align*}
Taking a union bound over $n$ vertices gives the result.
\end{proof} 




\begin{lemma}
\label{lem2} 
Fix $t\in \field{Z}^+$ and $0<\alpha<1$. Then, \whp there does not exist a subset $S \subseteq [n]$, 
such that $|S| \leq \alpha t L$ and $e[S] \geq |S|+t$. 
\end{lemma}

\begin{proof}
Set $s=|S|$.Then,
\begin{align*}
\Prob{ \exists S: s \leq \alpha t L \text{~~and~~} e[S] \geq s+t } 
&\leq \sum_{s \leq \alpha t L} \binom{n}{s} \binom{\binom{s}{2}}{s+t} p^{s+t}  \leq \sum_{s \leq \alpha t L } \bfrac{ne}{s}^s \bfrac{es^2p}{2(s+t)}^{s+t} \\ 
&\leq \sum_{s \leq \alpha t L } (e^{2+o(1)}\log{n})^s \bfrac{6es\log{n}}{n}^t \\
&\leq  \alpha tL \brac{ (e^{2+o(1)}\log{n})^{ \alpha L} \bfrac{6e \alpha t\log^2{n} }{n\log{\log{n}}}}^t < \frac{1}{n^{(1-\a-o(1))t}}.
\end{align*}
\end{proof}



\begin{lemma}
\label{lem3}
Let $T$ be a rooted tree of depth at most $\frac{4L}{7}$ and let $v$ be a vertex not in $T$.  Then with probability $1-o(n^{-3})$, $v$ has at most $10$ neighbors in $T$, i.e., $|N(v) \cap T| \leq 10$.
\end{lemma} 

\begin{proof}
Let $T$ be a rooted tree of depth at most $2L/3$ and let $S$ consist of $v$, the neighbors of $v$ in $T$ plus the ancestors of these neighbors. Then 
$|S|\leq 4bL/7+1\le 3bL/5$ and $e(S)=|S|+b-2$. It follows from Lemma \ref{lem2} with $\a=3/5$ and $t=8$, that 
we must have $b\leq 10$ with probability $1-o(n^{-3})$.
\end{proof} 

\noindent We show that by growing trees iteratively we can construct 
sufficiently many almost edge disjoint paths.  

\begin{figure*}[!ht]
\centering
\begin{tabular}{@{}c@{}@{\ }c@{}} \includegraphics[width=0.33\textwidth]{fig2.jpg}  \hspace{6mm} & \includegraphics[width=0.33\textwidth]{fig1.jpg} \\
(a) & (b)  
\end{tabular}
\caption{\label{fig:fig1} (a) By repeatedly growing trees  appropriately, (b) we create for each pair of nodes $x,y$ two node disjoint trees $T_x,T_y$ of depth $\diam\times \frac{1}{\sqrt{\log\log n} }$ whose leaves can be matched via a natural isomorphism and linked with edge disjoint paths of length $(1+o(1))\diam$}
\vspace{-4mm}
\end{figure*}



\begin{lemma}
\label{lem4} 
For all pairs of  vertices $x,y \in [n]$ there exists a subgraph $G_{x,y}(V_{x,y},E_{x,y})$ of $G$ as shown in figure~\ref{fig:fig1}, {\it whp}.
The subgraph consists of two isomorphic vertex disjoint trees $T_x,T_y$ rooted at $x,y$ each of depth $k$.
$T_x$ and $T_y$ both have a branching factor of $3\log n$.
If the leaves of $T_x$ are $x_1,x_2,\ldots,x_\tau,\tau\geq n^{4\epsilon/5}$ then $y_i=f(x_i)$ where $f$ is a natural 
isomporphism.
Between each pair of leaves $(x_i,y_i),i=1,2,\ldots,m$ 
there is a path $P_i$ of length  $(1+2\epsilon) L$. The paths $P_i,i=1,2,\ldots,\tau,\ldots$ are edge disjoint.
\end{lemma}


\begin{proof}
Because we have to do this for all pairs $x,y$, we note without further comment that likely (resp. unlikely) 
events will
be shown to occur with probability $1-o(n^{-2})$ (resp. $o(n^{-2}$)).

To find the subgraph shown in Figure~\ref{fig:fig1}(b) we grow tree structures as shown 
in Figure~\ref{fig:fig1}(a). 
Specifically, we first grow a tree from $x$ using BFS until it reaches  depth $k$. 
Then, we grow a tree starting from $y$ again using BFS until it reaches depth $k$. 
Finally, we grow trees from the leaves of $T_x$ and $T_y$ using BFS for depth $\gamma=(\frac{1}{2}+\epsilon)L$. 
Now we analyze these processes. Since the argument is the same we explain
it in detail for $T_x$ and we outline the differences for the other trees. 
We use the notation $D_i^{(\r)}$ for the number of vertices at depth $i$
of the BFS tree rooted at $\r$.



 

First we grow $T_x$. As we grow the tree via BFS from a vertex $v$ at depth $i$ to vertices 
at depth $i+1$ certain {\em bad} edges from $v$ may point 
to vertices already in $T_x$. Lemma \ref{lem3} shows with probability $1-o(n^{-3})$ there can be at most
10 bad edges emanating from $v$.

% Furthermore, 
%Lemma \ref{lem2} implies that there exists at most one vertex of degree less than $\frac{\log{n}}{100}$ 
%at each level {\it whp}. 
Hence, we obtain the recursion  

\beq{rec1}
D_{i+1}^{(x)} \geq \brac{5\log{n}-10} (D_i^{(x)}-1) \geq 4 \log{n}D_i^{(x)}.
\eeq

\noindent Therefore the number of leaves satisfies 

\beq{rec2}
D_{k}^{(x)} \geq \Big(4\log n\Big)^{\e L}\geq n^{4\e/5}.
\eeq
We can make the branching factor exactly $4\log n$ by pruning.
We do this so that the trees $T_x$ are isomorphic to each other. With a similar argument 
\beq{rec3}
D_{k}^{(y)} \geq n^{\frac{4}{5}\epsilon}.
\eeq
The only difference is that now we also say an edge is bad if the other endpoint is in $T_x$.
This immediately gives
$$D_{i+1}^{(y)} \geq \brac{5\log{n}-20} (D_i^{(y)}-1) \geq 4\log{n}D_i^{(y)}$$
and the required conclusion \eqref{rec3}.

Similarly, from each leaf $x_i \in T_x$ and $y_i \in T_y$ we grow trees $\hT_{x_i},\hT_{y_i}$ of depth 
$\gamma = \big(\frac{1}{2}+\epsilon\big) L$ using the same procedure and arguments 
as above. Lemma~\ref{lem3} implies that there are at most 20 edges from the vertex $v$ being explored to 
vertices in any of the trees already constructed. At most 10 to $T_x$ plus any trees rooted at an $x_i$ 
and another 10 for $y$.
The numbers of leaves of each $\hT_{x_i}$ now satisfies
$$\hD_\g^{(x_i)}\geq 5\log{n} (4\log{n})^{\g}\geq n^{\frac{1}{2}+\frac{4}{5}\epsilon}.$$
Similarly for $\hD_\g^{(y_i)}$.



\noindent Observe next that BFS does not condition the edges between the leaves $X_i,Y_i$ of the trees $\hT_{x_i}$ 
and $\hT_{y_i}$.
I.e., we do not need to look at these edges in order to carry out our construction. 
On the other hand we have conditioned on the occurence of certain events to imply a certain growth rate.
We handle this technicality as follows. We go through the above construction and halt if ever we find that we cannot
expand by the required amount. Let ${\bf A}$ be the event that we do not halt the construction
i.e. we fail the conditions of Lemmas \ref{lem2} or \ref{lem3}. We have
$\Prob{{\bf A}}=1-o(1)$ and so,
$$\Prob{\exists i:e(X_i,Y_i)=0\mid {\bf A}}\leq \frac{\Prob{\exists i:e(X_i,Y_i)=0}}{\Pr({\bf A})}\leq
2n^{\frac{4\e}{5}}(1-p)^{n^{1+\frac{8\e}{5}}}\leq n^{-n^\e}.$$
We conclude that {\em whp} there is always an edge between each $X_i,Y_i$ and thus a path of length at most
$(1+2\e)L$ between each $x_i,y_i$.
\end{proof}
 


The proof of Theorem~\ref{thm:thrm1} follows. For notational simplicity set $q=\frac{1}{2}-b$.

\begin{proof} 
Fix a pair of nodes $x,y \in V(G)$.  Let $Y_1,\ldots,Y_N$  be the signs of the $N$ edge  disjoint paths connecting them, i.e., $Y_i \in \{-1,+1\}$ for all $i$. Also let $Y= \sum_{i=1}^N Y_i$. Notice that $\{Y_1,\ldots,Y_N\}$ is a read-$k$ family where $k=\frac{N}{6\log{n}}$.  


% Suppose $f(x)=f(y)$. The case $f(x)\neq f(y)$ is worked out in an identical way and details are omitted.  
 Set  $r = \frac{1+(1-2q)^L}{2}$.  By the linearity of expectation $\Mean{Y} = N(2b)^L$. Let $\frac{1}{2e^{\tfrac{4}{5} \sqrt{\log\log{n}}}}\ll b$. Then

\begin{align*}
\Mean{Y} &= n^{\tfrac{4}{5}\epsilon} (2b)^{\frac{\log{n}}{\log\log{n}}} \geq  \exp\Bigg( \frac{4}{5} \frac{\log{n}}{\sqrt{\log\log{n}}} - \log{(\frac{1}{2b})} \frac{\log{n}}{\log\log{n}} \Bigg) \geq \exp\Bigg( (1-o(1)) \frac{4}{5} \frac{\log{n}}{\sqrt{\log\log{n}}}  \Bigg).
\end{align*}

By applying Theorem~\ref{thm:readk} we obtain  

\begin{align*}
\Prob{Y<0} &= \Prob{Y-\Mean{Y} < -\Mean{Y} } \leq \exp \Big( \frac{n^{4/5\epsilon}}{\frac{2n^{4/5\epsilon} }{4\log{n}}} \Big)=o(n^{-2}).
\end{align*}


\end{proof} 

 
